Sequential Decision Problems with Weak Feedback

This thesis considers sequential decision problems, where the loss/reward incurred by selecting an action may not be inferred from observed feedback. A major part of this thesis focuses on the unsupervised sequential selection problem, where one can not infer the loss incurred for selecting an action from observed feedback. We also introduce a new setup named Censored Semi Bandits, where the loss incurred for selecting an action can be observed under certain conditions. Finally, we study the channel selection problem in the communication networks, where the reward for an action is only observed when no other player selects that action to play in the round. These problems find applications in many fields like healthcare, crowd-sourcing, security, adaptive resource allocation, among many others. This thesis aims to address the above-described sequential decision problems by exploiting specific structures these problems exhibit. We develop provably optimal algorithms for each of these setups with weak feedback and validate their empirical performance on different problem instances derived from synthetic and real datasets.

==> chapter0/abbreviations.tex <==
%!TEX root =  ../thesis.tex


\chapter*{List of Abbreviations}
\label{ch:ListOfAbr}
\addcontentsline{toc}{chapter}{\nameref{ch:ListOfAbr}}

\makeatletter
\newcommand{\tocfill}{\cleaders\hbox{}\hfill}
%\newcommand{\tocfill}{\cleaders\hbox{$\m@th \mkern\@dotsep mu . \mkern\@dotsep mu$}\hfill}
\makeatother
\newcommand{\abbrlabel}[1]{\makebox[3cm][l]{\textbf{#1}\ \tocfill}}
\newenvironment{abbreviations}{\begin{list}{}{\renewcommand{\makelabel}{\abbrlabel}
                                              \setlength{\itemsep}{0pt}}}{\end{list}}
%\begin{abbreviations}[labelsep=1em,font=\bfseries]
\begin{abbreviations}
\item[AGU] 	Adaptive Generalized Unitary transformation
\item[API] Application Programming Interface
\item[BSC]	Backscattering Coefficient
\item[SAR]  Synthetic Aperture Radar  
\item[CTD]	Coherent Target Decomposition
\end{abbreviations}


==> chapter0/approval.tex <==
%!TEX root =  ../thesis.tex

\begin{center}
	{\LARGE \bf Thesis Approval}	
	\vspace{0.5in}
	
	{\large The thesis entitled}
	\vspace{0.2in}
	
	{\LARGE \bf Online Machine Learning with Limited Feedback}
	\vspace{0.2in}
	
	{\large by}
	\vspace{0.2in}
	
	{\Large \bf Arun Verma} \\
	{\Large (Roll No. 154190002)}
	\vspace{0.2in}
	
	{\large is approved for the degree of} 
	\vspace{0.2in}
	
	{\large Doctor of Philosophy}
	\vspace{0.5in}
\end{center}

%\vspace{0.2in}
\hspace{4.75cm} {\large $\overline{\text{  }}$} \hspace{6.3cm} {\large $\overline{\text{   }}$}

\hspace{3.4cm} {\Large(Examiner)} \hspace{3.7cm} {\Large(Examiner)}

\vspace{1in}

\hspace{2cm} {\Large $\overline{\text{Manjesh K. Hanawal}}$}  \hspace{2cm} {\Large $\overline{\text{N. Hemachandra}}$}

\hspace{3.3cm}{\Large(Supervisor)} \hspace{3cm} {\Large(Co-Supervisor)}

\vspace{0.5in}
\begin{center}
	{\large $\overline{\text{  }}$}\\
	{\Large(Chairman)}
\end{center}

\vspace{0.5in}
\noindent
{\Large Date:} \rule{4cm}{1sp} \\
{\Large Place:} \rule{4cm}{1sp}

%\noindent Date: \underline{\ \qquad\qquad\qquad \ } \\
%Place:  \underline{\ \qquad\qquad\qquad \ } 

==> chapter0/symbols.tex <==
%!TEX root =  ../thesis.tex


\chapter*{List of Symbols}
\label{ch:sym}
\addcontentsline{toc}{chapter}{\nameref{ch:sym}}
\makeatletter
%\newcommand{\tocfill}{\cleaders\hbox{$\m@th \mkern\@dotsep mu . \mkern\@dotsep mu$}\hfill}
\makeatother
%\newcommand{\abbrlabel}[1]{\makebox[3cm][l]{\textbf{#1}\ \tocfill}}
\newenvironment{symbols}
	{\begin{list}{}{
		\renewcommand{\makelabel}{\abbrlabel}
        \setlength{\itemsep}{0pt}}
    }{\end{list}}


\begin{symbols}
	\item[$\mu$] 	Rate	
\end{symbols}


==> chapter4/conclusion.tex <==
%!TEX root =  ../thesis.tex


We introduce a novel framework for resource allocation problems using a variant of semi-bandits and name it censored semi-bandits (CSB). In the CSB setup, the loss observed from an arm depends on the amount of resource allocated, and hence, it can be censored. We propose a threshold-based model where a loss from an arm is generated independently from a fixed and unknown distribution, but it is only observed when the allocated resource is below a threshold. The goal is to assign a given resource to arms such that total expected loss is minimized. We consider two variants of the problem, depending on whether or not the thresholds are the same across the arms. For the variant where thresholds are the same across the arms, we establish that its sub-problem is equivalent to the Multiple-Play Multi-Armed Bandit problem. For the second variant, where the threshold can depend on the arm, we establish that its sub-problem is equivalent to a more general Combinatorial Semi-Bandit problem. Exploiting these equivalences, we develop algorithms that enjoy optimal performance guarantees.  We also showcase the application of the CSB setup to stochastic network utilization maximization by extending the CSB setup to the reward maximization setting.


The CSB setting considered so far does not use any similarity metric between the arms. For example, in the case of the police patrol allocation, the nearby nodes may have similar parameters, and we may be able to make use of such spatial coherence. It will be interesting to integrate existing work on contextual bandits with the graph structure in the CSB setup. As we consider only one type of resource, it will be interesting to consider multi-type resources in the CSB setup. Another extension of the CSB setup is to relax the assumption that the lower bound on leftover resources after the optimal allocation is known. One can also extend the CSB setup from threshold type loss to continuous type loss functions and from the stochastic environment to the adversarial environment. 



